Fast Quantum Fourier Transforms for a Class of Non-abelian Groups

An algorithm is presented allowing the construction of fast Fourier transforms for any solvable group on a classical computer. The special structure of the recursion formula being the core of this algorithm makes it a good starting point to obtain systematically fast Fourier transforms for solvable groups on a quantum computer. The inherent structure of the Hilbert space imposed by the qubit architecture suggests to consider groups of order 2^n first (where n is the number of qubits). As an example, fast quantum Fourier transforms for all 4 classes of non-abelian 2-groups with cyclic normal subgroup of index 2 are explicitly constructed in terms of quantum circuits. The (quantum) complexity of the Fourier transform for these groups of size 2^n is O(n^2) in all cases.

==> pic/circ.tex <==
%\begin{picture}(40,120)(0,-10)
%\put(0,0){\line(1,0){40}}
%\put(0,20){\line(1,0){7}}
%\put(0,40){\line(1,0){7}}
%\put(0,60){\vdots}
%\put(0,80){\line(1,0){7}}
%\put(0,100){\line(1,0){7}}
%\put(7,10){\line(1,0){20}}
%\put(7,90){\line(1,0){20}}
%\put(7,10){\line(0,1){80}}
% 
%\put(0,0){\line(1,0){40}}
%\put(23,20){\line(1,0){7}}
%\put(23,40){\line(1,0){7}}
%\put(23,60){\vdots}
%\put(23,80){\line(1,0){7}}
%\put(23,100){\line(1,0){7}}
%\put(33,10){\line(1,0){20}}
%\put(33,90){\line(1,0){20}}
%\put(23,10){\line(0,1){80}}
% 
%\put(10,50){$U$}
% 
%\end{picture}

